The Surprising Benefits of Base Rate Neglect in Robust Aggregation

Robust aggregation integrates predictions from multiple experts without knowledge of the experts' information structures. Prior work assumes experts are Bayesian, providing predictions as perfect posteriors based on their signals. However, real-world experts often deviate systematically from Bayesian reasoning. Our work considers experts who tend to ignore the base rate. We find that a certain degree of base rate neglect helps with robust forecast aggregation. Specifically, we consider a forecast aggregation problem with two experts who each predict a binary world state after observing private signals. Unlike previous work, we model experts exhibiting base rate neglect, where they incorporate the base rate information to degree $\lambda\in[0,1]$, with $\lambda=0$ indicating complete ignorance and $\lambda=1$ perfect Bayesian updating. To evaluate aggregators' performance, we adopt Arieli et al. (2018)'s worst-case regret model, which measures the maximum regret across the set of considered information structures compared to an omniscient benchmark. Our results reveal the surprising V-shape of regret as a function of $\lambda$. That is, predictions with an intermediate incorporating degree of base rate $\lambda<1$ can counter-intuitively lead to lower regret than perfect Bayesian posteriors with $\lambda=1$. We additionally propose a new aggregator with low regret robust to unknown $\lambda$. Finally, we conduct an empirical study to test the base rate neglect model and evaluate the performance of various aggregators.

==> useless/exp_v1.tex <==

\section{Study}\label{study}

We have theoretically and numerically assessed the performance of different aggregators. Regarding aggregating predictions from real-world human subjects, we investigate the following questions:

\begin{itemize}
\item [(1)] Do people display base rate neglect as prior empirical studies suggest?

\item [(2)] Which aggregator is best for aggregating predictions empirically?

\item [(3)] Does a certain degree of base rate neglect help aggregation in practice?
\end{itemize}

To further examine these questions, we conduct an online study to identify base rate neglect in human subjects and empirically compare our aggregators with alternatives. To make our comparison more representative, we use average loss to measure aggregator's performance. Our findings are:

\begin{itemize}
\item [(1)] Very few are perfect Bayesians. Many display base rate neglect. However, around 60\% of predictions do not fall between perfect BRN and Bayes, beyond the theoretical framework. Around 16\% even just report the prior, indicating a tendency opposite to BRN. \yk{justification}

\item [(2)] For the general population, simple averaging achieves the lowest loss. This is because ~60\% of predictions fall outside the BRN-Bayes range our theory considers. When we restrict the predictions into the group that is inside the BRN-Bayes range, certain $\lambda$-base rate balancing aggregators can achieve lower loss than other aggregators, such as simple average and average prior, aligning with previous sections. \shu{whether our balancing aggregator includes average prior?}

\item [(3)] Within the inside group, some degree of base rate neglect does not necessarily hurt forecast aggregation - it may even improve it. 
\end{itemize}

We will now present the design and results of the study in detail. Different from previous studies that only focus on one specific information structure \citep{}\shu{some citations here, such as the AER paper}, an additional contribution of our work is that we collect a comprehensive dataset containing predictions under hundreds of information structures spanning the entire spectrum. 


\yk{highlight here for empirical data, we focus on a finite set of information structures. mostly focus on average case results. (perhaps also attach the numerical results for the average case)}\shu{add emphasis.}


\subsection{Study Design and Data Collection}
\label{section:design}

\paragraph{\textbf{Task}} We use the belief-updating task to elicit the forecast of participants. Specifically, there are two boxes, each of which contains a mix of red and blue balls with a maximum of 100 balls. In the left box, the proportions of red balls and blue balls are $p_l\in (0,1)$ and $(1-p_l)$, and in the right box the proportions are $p_r\in (0,1)$ and $(1-p_r)$. Moreover, the probability of selecting the left box is $\mu\in(0,1)$, and that of the right box is $1-\mu$. A ball is randomly drawn from the selected box as a signal. After knowing the color of the signal, participants are required to estimate the probability that the drawn ball comes from the left box.\footnote{Specifically, the two questions are ``If the ball is red, what is the probability that it comes from the left box'' and ``If the ball is blue, what is the probability that it comes from the left box''.} To collect individual predictions under different information structures as much as possible, we discretize each of the parameters in $\{p_l, p_r, \mu\}$ with increments of 0.1. Consequently, we construct an information structure set with $9\times9\times9=719$ cases, and each subject is required to answer 30 different cases. To enhance the independence of responses to questions conditional on the two signals within the same information structure, we randomly assign them across rounds. This approach yields a total of 60 rounds of questions for each subject. All predictions must be expressed as percentage points and fall within the range of 0\% to 100\%.

\paragraph{\textbf{Procedure}} The experiment is conducted using Otree \citep{chen2016otree} and we recruit a balanced sample of male and female from Prolific. Subjects provide informed consent and are made aware that their responses would be used for research purposes. We use the incentive-compatible BDM method \citep{becker1964measuring} to elicit their true belief.\footnote{Subjects can receive an additional bonus of either \$6 or \$0, depending on their decisions.} Additionally, we also introduce the example task and payment scheme before the formal task to guarantee subjects' understanding. Appendix \ref{appendix:instruction} shows the instructions to participants.

At last, 201 subjects finished the study. On average, there are 8.39 predictions under each information structure. The experiment lasts 33.74 minutes and the average payment is around \$8.16 (including \$5.5 participation fee).

\hide{At last, 201 subjects finished the study, and we exclude x of them who spent less than x minutes on the study, resulting in x subjects and x predictions used for the formal analyses. Thus, on average, there are x predictions under each information structure. The average duration for the remaining subjects is 33.7 minutes and the average payment is \$x.  }


%\section{Empirical Analysis of Base Rate Neglect in Humans}


\subsection{Identification of Base Rate Neglect}\label{subsection:brn}

The motivation of our work is the well-observed deviation from Bayesian predictions. Thus, we first aim to identify whether participants submit Bayesian responses in our study. Ideally, they should apply Bayes' rule to update their beliefs, and we can use perfect Bayes $x^{Bayes}(r) = \frac{\mu \cdot p_l}{\mu  \cdot p_l + (1-\mu)  \cdot p_r}$ and $x^{Bayes}(b) = \frac{\mu  \cdot (1-p_l)}{\mu  \cdot (1-p_l) + (1-\mu) \cdot  (1-p_r)}$ as benchmark, where $r$ and $b$ represent  the signal of red ball and blue ball, respectively. Furthermore, similar to \citet{esponda2023mental}\shu{improvement?}, we define responses that completely ignore prior and report $x^{pBRN}(r) = \frac{p_l}{p_l+p_r}$ and $x^{pBRN}(b) = \frac{1-p_l}{(1-p_l)+(1-p_r)}$ as perfect Base Rate Neglect (perfect BRN) with $\lambda = 0$ . 


\paragraph{\textbf{Base rate neglect at prediction level}} The results of our study show that only 9.14\% of predictions are consistent with perfect Bayes.\footnote{We exclude the case when $\mu = 0.5$ during the analyses in this subsection, because there is no difference between $x^{Bayes}$ and $x^{pBRN}$.}$^{,}$\footnote{We relax the Bayesian belief by permitting rounding $x^{Bayes}$ both up and down to two decimal places, and the same principle applies to $x^{pBRN}$.} 
Meanwhile, 4.66\% of predictions fully ignore the base rate, satisfying perfect BRN.\hide{called pure Base Rate Neglect (pure BRN)\shu{should we mention the abbreviation here again?}}
26.62\% of responses fall into the range between $x^{Bayes}$ and $x^{pBRN}$, and 59.58\% fall outside. We also notice that there are 16.20\% of predictions consistent with the prior. \yk{among the outside?}\shu{I am wondering whether to mention this proportion of q == mu, because it cannot be classified into either one of the above types.}
When we narrow our focus to the predictions in the first round instead of all 60 rounds, where learning effect is not a concern, the proportion of perfect Bayes slightly decreases, while that of perfect BRN slightly increases, both reaching 6.99\%. \yk{do not understand this sentence, red ball round?}\shu{more clear now maybe.} 


Figure~\ref{fig: ans_ratio} shows the proportion of different types of responses conditional on the signal across rounds. We observe that these proportions are relatively stable with respect to both rounds and signals.\hide{Further details are shown in Appendix\hide{~\ref{appendix:analyses}}.} These findings illustrate that subjects' rarely submit Bayesian beliefs. 

\yk{change notations here}\shu{changed}

\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{picture/ratio.pdf}
    \caption{The Proportion of Different Types of Response}
    \label{fig: ans_ratio}
\begin{flushleft}
{\footnotesize \textit{Notes:} We exclude the responses when $\mu=50$. Panel A and B present the responses when the signal is red and blue, respectively. \hide{Red solid line denotes the proportion of responses that equal to $B_{Bay}$, blue dash line denotes that equal to $B_{pBRN}$, green dash-dot line indicates that fall between the two, and brown line indicates that fall outside.}}
\end{flushleft}
\end{figure}

\paragraph{\textbf{Base rate neglect at subject level}} After exploring base rate neglect at prediction level, another question arises: how far do subjects deviate from Bayesians? To answer this question, we estimate the consideration degree of base rate, $\lambda$,  for each subject $i$. According to Observation \ref{lemma: BNR prediction vs Bayesian}, we can obtain the following econometric model, 

\[\logit (x^{Bayes}_t) - \logit (x_{t}) =\beta \cdot \logit(\mu_{t}) + \varepsilon_{t} \]

where $t$ indexes round, and $\logit(x)$ represents $\log \frac{x}{1-x}$. The coefficient $\beta$ is of our interest, and $\lambda = 1- \beta$. We estimate the above equation using OLS for each subject, and Figure \ref{fig: est_lambda} depicts the distribution of estimated $\lambda_i$. The results show that $\lambda_i$ exhibits three peaks with nearly equal frequencies, corresponding to 0 (perfect BRN), 0.6 (moderate BRN), and 1 (perfect Bayes), respectively. The average consideration degree of base rate at subject level is 0.43, and it is also comparable to the estimate based on predictions of all subjects across all rounds, which is 0.44. Besides, there are some subjects whose $\lambda_i$ fall outside the range of $[0,1]$, but the deviation is not large and the proportion is relatively low, with only 2.99\% of $\lambda_i$ being smaller than -0.2. Here we note that our theoretical model cannot account for these outside cases, however, subsequent empirical analyses will complement this limitation by incorporating them.

\begin{figure}[h]
    \centering
    \includegraphics[width=0.4\linewidth]{picture/lambda_density.pdf}
    \caption{The Distribution of Estimated $\lambda_i$}
    \label{fig: est_lambda}
\begin{flushleft}
{\footnotesize \textit{Notes:} We exclude the responses when $\mu=50$. The red line signals the estimated $\lambda$ using predictions of all subjects.}
\end{flushleft}
\end{figure}

\yk{change notations, also explain that our model does not capture the outside case.... }


\subsection{Aggregator evaluation}

Conditional on the observed base rate neglect, we will further explore the performance of aggregators under subjects' predictions. According to Lemma \ref{lemma: square relative loss}, the relative loss of two information structures ($\theta_1,\theta_2$) that share the same prior ($\mu$), i.e., conditional independent information structures, can be calculated as follows.






\begin{comment}
\begin{equation*}
    Loss_{\theta_1,\theta_2}^{f} = \frac{\sum_{i\neq j, i\in \mathcal{I}_{\theta_1},j\in\mathcal{I}_{\theta_2}}\sum_{s_i, s_j \in \{ r, b \}}
    \Pr(s_i,s_j)
\left[ f \left( x_i^{\theta}(s_i),  x_j^{\theta}(s_j)\right) - f^*\left(s_i, s_j\right) \right]^2  }{C_{|\mathcal{I}_{\theta}|}^{2}}
\end{equation*}
\end{comment}

\[Loss_{\theta_1,\theta_2}^{f} = 
\begin{cases} 
  \frac{\sum_{ i\in \mathcal{I}_{\theta_1}, j\in\mathcal{I}_{\theta_2},i\neq j}\sum_{s_i, s_j \in \{ r, b \}}
    \Pr(s_i,s_j)
\left[ f \left( x_i^{\theta_1}(s_i),  x_j^{\theta_2}(s_j)\right) - f^*\left(s_i, s_j\right) \right]^2  }{\sum_{ i\in \mathcal{I}_{\theta_1}, j\in\mathcal{I}_{\theta_2},i\neq j}1}, 
& \text{if } \theta_1 \neq  \theta_2  \\
  \frac{\sum_{i,j\in \mathcal{I}_{\theta},i < j}\sum_{s_i, s_j \in \{ r, b \}}
    \Pr(s_i,s_j)
\left[ f \left( x_i^{\theta}(s_i),  x_j^{\theta}(s_j)\right) - f^*\left(s_i, s_j\right) \right]^2  }{\sum_{i,j\in \mathcal{I}_{\theta},i < j} 1}, & \text{if } \theta_1 = \theta_2 =\theta .
\end{cases}
\]

\begin{equation*}
\text{where }
 f^*(s_i,s_j)=  \frac{\mu\cdot\Pr[s_i\mid \omega = 1]\cdot \Pr[s_j\mid \omega = 1]}{\mu\cdot\Pr[s_i\mid \omega = 1]\cdot \Pr[s_j\mid \omega = 1] + (1-\mu)\cdot \Pr[s_i\mid \omega = 0]\cdot \Pr[s_j\mid \omega = 0]}
\end{equation*}
\hide{One mu may be answered by one subject more than once. But we use $\theta$ to indicate, which is information structure and it is identical to subjects.}
In the above equation, $i$ and $j$ index subjects.\hide{ $r$ represents the selected ball is in red, and $b$ represents that in blue. } $\mathcal{I}_{\theta}$ defines the set of subjects who predict under information structure $\theta$.\hide{, and $|\mathcal{I}_{\theta}|$ is the number of elements in $\mathcal{I}_{\theta}$. } Intuitively, $Loss$ is measured by the square relative loss of pairwise \hide{non-repeating}combinations of predictions under the information structures. On a related note, to guarantee the independence of predictions and avoid aggregating the two predictions from the same subject, we exclude the cases where $i=j$ under different information structures. Moreover, we also eliminate the repeated combinations under the same information structure, because $f \left( x_i^{\theta}(s_i),  x_j^{\theta}(s_j)\right) 
 = f \left( x_j^{\theta}(s_j),  x_i^{\theta}(s_i)\right) $.\footnote{Note that one subject cannot face the same information structure due to our assignment rule.}

Thus, we can construct a dataset uniquely identified by information structure $\theta_1,\theta_2$,\hide{, aggregator $f$ and pairwise non-repeating combination indexed by subjects $i$ and $j$. } which enables us to formally evaluate the performance of aggregators. To calculate the relative loss of aggregators under Bayesian posterior, we replace $ f \left( x_i(s_i),  x_j(s_j)\right)$ with $ f \left( x^{Bayes}(s_i), x^{Bayes}(s_j)\right)$.

%\paragraph{\textbf{Overall performance}}
\paragraph{\textbf{Whole sample analyses}}
Panel A in Tables \ref{table:agg perf} summarizes the performance of simple average and average prior, and Panel B summarizes that of our $\lambda$-base rate balancing aggregators. We find that when $\hat{\lambda}$ ranges from 0.1 to 0.9, both the average loss and maximum loss of aggregating subjects' predictions decrease (Column 1-2), and all these aggregators perform worse than average prior and simple average, where simple average achieves the lowest average loss. The same trend applies to aggregating Bayesian posterior when $\hat{\lambda}$ changes, except that the $\lambda$-base rate balancing aggregator with $\hat{\lambda}=0.9$ outperforms average prior regarding average loss, and simple average aggregator only show a medium-level performance.


\hide{
\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{picture/diff_density.pdf}
    \caption{PDF of the Difference of Loss between Subjects' predictions and Bayesian Posteriors}
    \label{fig: diff_density}
\begin{flushleft}
{\footnotesize \textit{Notes:} \shu{change the color as figure 4\&7} }
\end{flushleft}
\end{figure}
}
\begin{table}[h]
\footnotesize
\begin{threeparttable}   
\begin{tabular}{lccccccc}
\hline \hline
 & \multicolumn{2}{c}{Subjects' predictions} & \multicolumn{2}{c}{Bayesian posteriors}& & \multicolumn{2}{c}{\% \textit{Loss}(Sub) < \textit{Loss}(Bay)} \\
 & \makecell{Average \\ loss} & \makecell{Maximum \\ loss} & \makecell{Average \\ loss} & \makecell{Maximum \\ loss} & \makecell{Diff. of loss \\ (1)-(3)} & \makecell{Information \\structure} & \makecell{Pair of \\predictions} \\
 & (1)&(2)  &(3)  & (4) &(5)  &(6) &(7) \\
 \hline
\multicolumn{8}{l}{\textit{Panel A: Previous Aggregators}} \\
Simple average & 0.0671 & 0.1867 & 0.0101 & 0.0392 & 0.0570 & 0.00 & 2.90 \\
Average prior & 0.0681 & 0.1957 & 0.0082 & 0.0209 & 0.0599 & 0.00 & 4.51 \\
\multicolumn{8}{l}{\textit{Panel B: $\lambda$-base rate balancing aggregators $f^{\hat{\lambda}}_{ap}$}} \\
$\hat{\lambda}=0.1$ & 0.0906 & 0.2656 & 0.0213 & 0.0483 & 0.0693 & 0.58 & 23.91 \\
$\hat{\lambda}=0.2$ & 0.0879 & 0.2581 & 0.0195 & 0.0444 & 0.0684 & 0.40 & 22.98 \\
$\hat{\lambda}=0.3$ & 0.0850 & 0.2502 & 0.0176 & 0.0405 & 0.0674 & 0.26 & 21.77 \\
$\hat{\lambda}=0.4$ & 0.0822 & 0.2425 & 0.0156 & 0.0366 & 0.0666 & 0.15 & 20.35 \\
$\hat{\lambda}=0.5$ & 0.0792 & 0.2345 & 0.0136 & 0.0326 & 0.0656 & 0.06 & 18.59 \\
$\hat{\lambda}=0.6$ & 0.0764 & 0.2262 & 0.0117 & 0.0286 & 0.0647 & 0.03 & 16.51 \\
$\hat{\lambda}=0.7$ & 0.0736 & 0.2177 & 0.0099 & 0.0251 & 0.0637 & 0.01 & 13.80 \\
$\hat{\lambda}=0.8$ & 0.0712 & 0.2102 & 0.0085 & 0.0235 & 0.0627 & 0.01 & 10.41 \\
$\hat{\lambda}=0.9$ & 0.0692 & 0.2029 & 0.0077 & 0.0220 & 0.0615 & 0.01 & 6.90 \\
Observations & 14,364 & 14,364 & 14,364 & 14,364 & 14,364 & 14,364 & 2,009,650 \\
\hline \hline
\end{tabular}
\begin{tablenotes}[flushleft]
\footnotesize \item \textit{Notes:} For the convenience of comparison, we exclude 12 pairs of predictions which cannot be aggregated by average prior aggregator or $\lambda$-base rate balancing aggregators, such as one subject has a report of 0\% while another have a report of 100\%. The same exclusion criterion applies to the following analyses.
\end{tablenotes}
\end{threeparttable}
\caption{Summary of Aggregator Performance}
\label{table:agg perf}
\end{table}

%\paragraph{\textbf{Subsample performance}}
\paragraph{\textbf{Subsample analyses}}
We notice that there exists a gap between our theoretical framework and the above empirical analyses. Theoretically, the consideration degree of base rate $\lambda$ ranges from 0 to 1, which means the actual prediction should be located between perfect BRN and perfect Bayes. However, as reported in Figure \ref{fig: ans_ratio}, around 60\% of predictions fall outside the range.\hide{, which may cause the aforementioned gap. }
Therefore, we divide the sample according to the relationship with the expected range and investigate the heterogeneous performance of our $\lambda$-base rate balancing aggregators, especially those within the perfect BRN - Bayes range.

As noticed in subsection \ref{subsection:brn}, there are two main types of predictions, which fall inside the outside the above range. In the forecast aggregation, we need to aggregate predictions from two experts and each expert provides two reports conditional on the signals. Thus, we consider 5 groups of subsample according to the composition of the 4 reports, ranging from 4 outsides reports to 4 inside reports.\hide{1) 4 outside reports, 2) 3 outside reports and 1 inside reports, 3) 2 outside reports and 2 inside reports, 4) 1 outside reports and 3 inside reports, 5) 4 inside reports. }
Additionally, we also consider 2 special cases, which are 4 prefect BRN and 4 perfect Bayes reports. Figure~\ref{fig: heter_agg} shows the performance of various aggregators across above subsample measured by average loss at the information structure level.

\input{picture/heter_agg}

For the cases of 4 outside reports and 1 inside and 3 outside reports, we find that simple average can achieve the lowest loss. However, it is not the same for other cases. Some $\lambda$-base rate balancing aggregator with $0< \hat{\lambda} < 1$ can surprisingly benefit the aggregation when most reports exhibit BRN, such as in the cases of 2 inside and 2 outside reports ($ \hat{\lambda} =0.9$ performs best), 3 inside and 1 outside reports ($ \hat{\lambda} =0.7$ performs best), 4 perfect BRN reports and 4 inside reports ($ \hat{\lambda} =0.5$ performs best). While for 4 perfect Bayes reports, average prior aggregator wins. The above findings emphasize the importance of selecting appropriate aggregators based on experts' consideration degree of the base rate, which can improve the accuracy of forecast aggregation. More importantly, our $\lambda$-base rate balancing aggregators excel in 4 out of 7 cases.

\subsection{Base Rate Neglect vs. Bayesian}

At last, we investigate the role of base rate neglect in forecast aggregation. Namely, given the same aggregator, we study whether consideration degree of base rate influences the performance of the aggregator. We know that subjects do not submit Bayesian beliefs.
Thus, we can compare the relative loss of an aggregator under two scenarios to answer this question, where the first is subjects' reports and the second is Bayesian posteriors. 

\paragraph{\textbf{Whole sample analyses}}
The classical aggregators including simple average and average prior achieve higher loss for human subjects (Column 5 in Table~\ref{table:agg perf}, Panel A). The average loss is 0.0671 and 0.0681 when aggregating all subjects' predictions for simple average and average prior (Column 1), while it decreases to 0.0101 and 0.0082 when aggregating Bayesian posteriors (Column 3). Meanwhile, in all information structures, Bayesian posteriors always benefit forecast aggregation (Column 7). 
%Additionally, we also find that average prior achieves higher loss when aggregating subjects' predictions while lower loss when aggregating Bayesian posteriors, compared to simple average.
%\footnote{We report relative loss at the information structure level in Table \ref{table:agg perf}, and we also summarize the performance at the level of prediction pairs in Table \ref{table:agg perf at pairs}. The findings remain unchanged.} 

As for $\lambda$-base rate balancing aggregators, base rate neglect also results in worse performance in general population (Column 5 in Table~\ref{table:agg perf}, Panel B). Moreover, the difference of relative loss decreases as $\hat{\lambda}$ increases (Column 3 in Table~\ref{table:agg perf}), indicating the performance of aggregating subjects' predictions getting better.\hide{ The distributions also shift towards left for larger $\hat{\lambda}$ (Panel B of Figure~\ref{fig: diff_density}).}
However, the proportion of achieving lower loss for subjects' predictions across information structure surprisingly decreases from 0.58\% to 0.01\% (Column 6) as $\hat{\lambda}$ increases. The change becomes even larger, from 23.92\% to 6.90\% (Column 7), when we consider the loss at the level of prediction pair instead of information structure. It reveals that there are some cases that aggregating non-Bayesian predictions achieves a lower loss than Bayesian ones, and the phenomenon is more pronounced for our $\lambda$-base rate balancing aggregators with lower $\hat{\lambda}$.

%In addition to the previous two aggregators, we further investigate the performance of our $\lambda$-base rate balancing aggregators, and compare them to simple average and average prior aggregators. The resultes are summarized in Panel B in Table~\ref{table:agg perf}.

%We find that when $\hat{\lambda}$ ranging from 0.1 to 0.9, both the average loss and maximum loss of aggregating subjects predictions decrease (Column 1-2), and all aggregators perform worse than average prior, where $\hat{\lambda}=1$, and simple average acheives the lowest average loss. The same trend applies to aggregating Bayesian predictions when $\hat{\lambda}$ changes, except that the $\lambda$-base rate balancing aggregator with $\hat{\lambda}=0.9$ outperform average prior regarding average loss, and simple average aggregator only show a medium-level performance.

\paragraph{\textbf{Subsample analyses}}
When comparing aggregators' performance in subgroup in Figure~\ref{fig: heter_agg}, we surprisingly find that 4 perfect Bayes reports does not always achieve lowest loss under different aggregators. Our aggregators with $ \hat{\lambda} <= 0.7$ can even achieve lower loss when aggregating 4 inside reports, compared to 4 perfect Bayes ones. Moreover, regardless of the type of aggregators, the lowest loss of aggregating 4 inside reports ($ \hat{\lambda} = 0.5$, $loss = 0.0070$) is smaller than aggregating 4 perfect Bayes (average prior with $ \hat{\lambda}= 1$, $loss = 0.0082$), which suggests base rate neglect does not necessarily compromise aggregation performance.

%Discussion of predictions outside perfect BRN - Bayes range
%k\subsection{Aggregator Performance on Human Data}

%Panel A in Figure \ref{fig: diff_density} presents the distribution of difference of relative loss between subjects' predictions and their Bayesian counterparts. 








%\subsubsection{Overall Performance}

%Simple averaging beats theory on full dataset
%\subsubsection{Performance Within BRN-Bayes Range}

%base rate balancing best for BRN-Bayes predictions

%Performance can benefit from some BRN






\begin{table}[h]
\footnotesize
\begin{threeparttable}   
\begin{tabular}{lccccccc}
\hline \hline
 & \multicolumn{2}{c}{Subjects' predictions} & \multicolumn{2}{c}{Bayesian posteriors}& & \multicolumn{2}{c}{\% \textit{Loss}(Sub) < \textit{Loss}(Bay)} \\
 & \makecell{Average \\ loss} & \makecell{Maximum \\ loss} & \makecell{Average \\ loss} & \makecell{Maximum \\ loss} & \makecell{Diff. of loss \\ (1)-(3)} & \makecell{Information \\structure} & \makecell{Pair of \\predictions} \\
 & (1)&(2)  &(3)  & (4) &(5)  &(6) &(7) \\
 \hline
\multicolumn{8}{l}{\textit{Panel A: Previous Aggregators}} \\
Simple average & 0.0627 & 0.2155 & 0.0091 & 0.0400 & 0.0536 & 0.00 & 3.19 \\
Average prior & 0.0638 & 0.2203 & 0.0076 & 0.0210 & 0.0562 & 0.00 & 4.80 \\
\multicolumn{8}{l}{\textit{Panel B: $\lambda$- base rate balancing aggregator $f^{\hat{\lambda}}_{ap}$}} \\
$\hat{\lambda}=0.1$ & 0.0882 & 0.2929 & 0.0225 & 0.0488 & 0.0657 & 0.71 & 25.20 \\
$\hat{\lambda}=0.2$ & 0.0853 & 0.2863 & 0.0205 & 0.0450 & 0.0648 & 0.49 & 24.25 \\
$\hat{\lambda}=0.3$ & 0.0823 & 0.2792 & 0.0184 & 0.0411 & 0.0639 & 0.34 & 23.00 \\
$\hat{\lambda}=0.4$ & 0.0793 & 0.2714 & 0.0163 & 0.0371 & 0.0630 & 0.22 & 21.53 \\
$\hat{\lambda}=0.5$ & 0.0762 & 0.2630 & 0.0141 & 0.0330 & 0.0621 & 0.14 & 19.66 \\
$\hat{\lambda}=0.6$ & 0.0731 & 0.2539 & 0.0120 & 0.0289 & 0.0611 & 0.07 & 17.52 \\
$\hat{\lambda}=0.7$ & 0.0702 & 0.2443 & 0.0100 & 0.0254 & 0.0602 & 0.03 & 14.69 \\
$\hat{\lambda}=0.8$ & 0.0675 & 0.2341 & 0.0083 & 0.0237 & 0.0592 & 0.01 & 11.10 \\
$\hat{\lambda}=0.9$ & 0.0652 & 0.2269 & 0.0073 & 0.0221 & 0.0579 & 0.00 & 7.36 \\
Observations & \multicolumn{1}{c}{29,889} & \multicolumn{1}{c}{29,889} & \multicolumn{1}{c}{29,889} & \multicolumn{1}{c}{29,889} & 29,889 & \multicolumn{1}{c}{29,889} & \multicolumn{1}{c}{4,218,968}
 \\
\hline \hline
\end{tabular}
\begin{tablenotes}[flushleft]
\footnotesize \item \textit{Notes:} For the convenience of comparison, we exclude 44 pairs of predictions which cannot be aggregated by average prior aggregator or $\lambda$-base rate balancing aggregators, such as one subject has a report of 0\% while another have a report of 100\%. The same exclusion criterion applies to the following analyses.
\end{tablenotes}
\end{threeparttable}
\caption{Summary of Aggregator Performance}
\label{table:agg perf}
\end{table}


==> useless/table_revise.tex <==
\paragraph{\textbf{Whole sample analyses}}
The classical aggregators including simple average and average prior achieve higher loss for human subjects (Column 5 in Table~\ref{table:agg perf}, Panel A). The average loss is 0.0627 and 0.0638 when aggregating all subjects' predictions for simple average and average prior (Column 1), while it decreases to 0.0091 and 0.0076 when aggregating Bayesian posteriors (Column 3). Meanwhile, in all information structures, Bayesian posteriors always benefit forecast aggregation (Column 7). 



As for $\lambda$-base rate balancing aggregators, base rate neglect also results in worse performance in general population (Column 5 in Table~\ref{table:agg perf}, Panel B). Moreover, the difference of relative loss decreases as $\hat{\lambda}$ increases (Column 3 in Table~\ref{table:agg perf}), indicating the performance of aggregating subjects' predictions getting better.\hide{ The distributions also shift towards left for larger $\hat{\lambda}$ (Panel B of Figure~\ref{fig: diff_density}).}
However, the proportion of achieving lower loss for subjects' predictions across information structure surprisingly decreases from 0.71\% to 0.00\% (Column 6) as $\hat{\lambda}$ increases. The change becomes even larger, from 25.20\% to 7.36\% (Column 7), when we consider the loss at the level of prediction pair instead of information structure. It reveals that there are some cases that aggregating non-Bayesian predictions achieves a lower loss than Bayesian ones, and the phenomenon is more pronounced for our $\lambda$-base rate balancing aggregators with lower $\hat{\lambda}$.


\paragraph{\textbf{Whole sample analyses}}
Panel A in Tables \ref{table:agg perf} summarizes the performance of simple average and average prior, and Panel B summarizes that of our $\lambda$-base rate balancing aggregators. We find that when $\hat{\lambda}$ ranges from 0.1 to 0.9, both the average loss and maximum loss of aggregating subjects' predictions decrease (Column 1-2), and all these aggregators perform worse than average prior and simple average, where simple average achieves the lowest average loss. The same trend applies to aggregating Bayesian posterior when $\hat{\lambda}$ changes, except that the $\lambda$-base rate balancing aggregator with $\hat{\lambda}=0.9$ outperforms average prior regarding average loss, and simple average aggregator only shows a medium-level performance.


==> useless/useless.tex <==
We further regress the prediction 
Regression results shown in Column x in Table x also confirm that the predictions are not Bayesian. Moreover, the result is robust to a series of checks including 1) clustering the standard errors by the individual level to consider the intercorrelation of predictions within subject (Column x in Table x), 2) controlling for the round fixed effect to eliminate the learning effect \citep{esponda2023mental} (Column x in Table x), and 3) controlling for demographic characteristics to reduce the problem from omitted variables (Column x in Table x). The above findings provide consistent evidence of BRN, which further emphasize the importance of considering the degree of BRN when aggregating the predictions.



\begin{equation*}
    Loss_{i,j,\theta}^{f} = \frac{\sum_{i\neq j\in \mathcal{I}_{\theta}}\sum_{s_i \in \{ r, b \}}\sum_{s_j \in \{ r, b \}} 
    \Pr(s_i)\Pr(s_j)
\left[ f \left( x_i^{\theta}(s_i),  x_j^{\theta}(s_j)\right) - f^*\left(s_i, s_j\right) \right]^2  }{C_{|\mathcal{I}_{\theta}|}^{2}}
\end{equation*}


\begin{equation*}
    Loss_{i,j,\theta}^{f} = \sum_{s_i \in \{ r, b \}}\sum_{s_j \in \{ r, b \}} 
    \Pr(s_i,s_j)
\left[ f \left( x_i^{\theta}(s_i),  x_j^{\theta}(s_j)\right) - f^*\left(s_i, s_j\right) \right]^2  
\end{equation*}


\textcolor{red}{Robust aggregation involves aggregating predictions from multiple experts. However, most existing studies assume that experts adhere to Bayesian principle, overlooking the well-documented phenomenon of base rate neglect. Our work builds on and extends the framework introduced by \citet{arieli2018robust} to incorporate the consideration degree of base rate ($\lambda$) and find it benefits the accuracy of forecast aggregation.}

\textcolor{red}{In our theoretical model, we reveal that any aggregator should exhibit a non-monotonic V-shaped regret regarding $\lambda$. Specifically, the aggregator may achieve lower regret when the experts exhibit base rate neglect, compared to Bayesian experts.
We further propose a family of aggregators with embedded fixed consideration degree of base rate, which theoretically (?) outperform classical aggregators such as simple average and average prior. In addition to theoretical analyses, we also conduct a study to collect predictions across hundreds of discrete information structures to empirically evaluate the performance of various aggregators.}


When considering our extended average prior aggregator with different $\lambda$ in Panel B, there are two observations.
First, as $\lambda$ increases, there is a lower likelihood of outperforming aggregation with Bayesian posteriors.
Second, as $\lambda$ increases, the relative loss difference becomes less pronounced. Table \ref{table:agg perf} also provides consistent findings. The difference of relative loss decreases from 0.0693 to 0.0615 when $\hat{\lambda}$ increases from 0.1 to 0.9. 

Meanwhile, the probability of achieving lower loss for subjects' predictions decreases from 0.58\% to 0.01\% (Column 5). The change becomes even larger, from 23.92\% to 6.90\% (Column 6), when we consider the loss at the level of prediction pair instead of information structure. \shu{It indicates that though the extended average prior with higher $\hat{\lambda}$ achieve---how to discuss? 1) the next step, separate different subjects using k or their answer. 2) discuss the performance of different aggregators.}



we aim to explore whether $f_{ap}^\lambda$ can achieve better performance than two alternative aggregators, simple average aggregator and average prior aggregator.  For $f_{ap}^\lambda$, we consider 9 specific aggregators with $\lambda \in \{0.1,0.2,...,0.8,0.9\}$. Under each information structure $\theta$, we evaluate the performance of each aggregator $f$ using square relative loss. According to 

\hide{
\begin{equation*}
\text{where}
\left\{
\begin{aligned}
  \  & \Pr[s=r] =  \mu \cdot p_l + (1-\mu )\cdot p_r \\
 & \Pr[s=b] = 1- \Pr[s=r]  \\
& f^*(s_i,s_j)=  \frac{\mu\cdot\Pr[s_i\mid \omega = 1]\cdot \Pr[s_j\mid \omega = 1]}{\mu\cdot\Pr[s_i\mid \omega = 1]\cdot \Pr[s_j\mid \omega = 1] + (1-\mu)\cdot \Pr[s_i\mid \omega = 0]\cdot \Pr[s_j\mid \omega = 0]}
\end{aligned}
\right.
\end{equation*}
}



\begin{equation*}
    Loss_{i,j,\theta}^{f} = \alpha + \beta \cdot Robust\_f_{i,j,\theta} +\tau_i + \psi_j+ \phi_{\theta} + \varepsilon_{i,j,\theta}^{f}
\end{equation*}

$Robust\_f$ is a dummy variable which denotes our aggregator. When the observation is generated by $f_{ap}^{\lambda}$, $Robust\_f$ equals to 1. We control for individual fixed effects $\tau_i$ and $\psi_j$, as well as fixed effect for information structure $\phi_{\theta}$, which capture unobservable factors. The error term $\varepsilon_{i,j,\theta}^{f}$ is clustered at the level of the information structure. To conduct pairwise comparison, we only use the subset generated by the two compared aggregators. In this way, $\beta$ represents the difference of loss between $f_{ap}^{\lambda}$ and alternative aggregator. According to our numeric simulation, we expect $\beta<0$, which means our aggregator can achieve lower loss than the others.

Table ? show the regression results. Panel A compares $f_{ap}^{\lambda}$ and simple average aggregator, and Panel B compares $f_{ap}^{\lambda}$ and average prior aggregator. From column 1 to 9, $\lambda$ ranges from 0.1 to 0.9 with increasement of 0.1. We find that . The above results are robust when we further control for round fixed effect for the two predictions. 
\shu{Then link to the theoretical part, which theorem can explain the result. Speak to ?}





\begin{figure}[h]
    \centering
    \includegraphics[width=0.85\linewidth]{picture/heter_agg.pdf}
    \caption{Aggregator performance in Subsample}
    \label{fig: est_lambda}
\begin{flushleft}
{\footnotesize \textit{Notes:} We exclude the responses when $\mu=50$. The red line signals the estimated $\lambda$ using all subjects.}
\end{flushleft}
\end{figure}







\begin{figure}[h]
    \centering
    \begin{tikzpicture}[scale=1.0] % Adjust the scale to increase or decrease the figure size
    \begin{axis}[
        width=\textwidth, % Adjust the width of the plot
        height=8cm, % Adjust the height of the plot
        xlabel={Aggregators},
        ylabel={Relative loss},
        xmin=1, xmax=11,
        xtick={1,2,3,4,5,6,7,8,9,10,11}, % 设置横坐标刻度的位置
        xticklabels={$\hat{\lambda}=0.1$, $\hat{\lambda}=0.2$, $\hat{\lambda}=0.3$, $\hat{\lambda}=0.4$, $\hat{\lambda}=0.5$, $\hat{\lambda}=0.6$, $\hat{\lambda}=0.7$, $\hat{\lambda}=0.8$, $\hat{\lambda}=0.9$, Avg. prior, Simp. avg.} , % 设置横坐标刻度标签的内容
        ytick={0.05,0.1,0.15}, % 设置横坐标刻度的位置
        yticklabels={0.05,0.1,0.15} , % 设置横坐标刻度标签的内容
        xticklabel style={rotate = 20},
        ymin=0, ymax=0.18,
        legend style={at={(0.5,-0.3)},
	       anchor=north,legend columns=3},
        grid style=dashed,
        ]

    %because I cannot cancel the point drawn and plot the star as the minimum point, thus I try to plot the line twice, and add the points afterwards.
    
    % 4 outside
    % plot the lie 
    \addplot[color=blue4,
    solid,
    line width=1pt,
    mark=diamond,
    mark options={solid},
    mark size=2.5pt] coordinates {
        (1.0,0.161691) (2.0,0.157436) (3.0,0.152885) (4.0,0.148020) 
    };
    \addlegendentry{4 outside}
    \addplot[color=blue4,
    solid,
    line width=1pt,
    mark=none,
    mark options={solid},
    mark size=2.5pt,
    forget plot] coordinates {
        (4.0,0.148020) (5.0,0.142828) (6.0,0.137306) (7.0,0.131467) (8.0,0.125350) (9.0,0.119046) (10.0,0.112732)
    };    
    %plot the ponits except for the minimum one
    \addplot[only marks, mark=diamond,color=blue4,mark size=2.5pt,line width=1pt, forget plot] coordinates {
     (5.0,0.142828) (6.0,0.137306) (7.0,0.131467) (8.0,0.125350) (9.0,0.119046) (11.0,0.106107)
    };
    %plot the minimum
    \addplot[only marks, mark=star,color=blue4,mark size=4pt,line width=1pt, forget plot] coordinates {
     (10.0,0.112732)
    };    

    % 1 bet + 3 outside
    \addplot[color=blue3,
    solid,
    line width=1pt,
    mark=o,
    mark options={solid},
    mark size=2.5pt] coordinates {
        (1.0,0.123774)(2.0,0.120498)(3.0,0.117073)(4.0,0.113511)
    };
    \addlegendentry{1 between + 3 outside}
    \addplot[color=blue3,
    solid,
    line width=1pt,
    mark=none,
    mark options={solid},
    mark size=2.5pt,forget plot] coordinates {
        (4.0,0.113511)(5.0,0.109834)(6.0,0.106079)(7.0,0.102311)(8.0,0.098630)(9.0,0.095199)(10.0,0.092275)
    };
    \addplot[only marks, mark=o,color=blue3,mark size=2.5pt,line width=1pt,forget plot] coordinates {
     (4.0,0.113511)(5.0,0.109834)(6.0,0.106079)(7.0,0.102311)(8.0,0.098630)(9.0,0.095199)(11.0,0.087503)
    };    
    \addplot[only marks, mark=star,color=blue3,mark size=4pt,line width=1pt,forget plot] coordinates {
     (10.0,0.092275)
    };    

    
    % 2 bet (2 subject) + 2 outside (2 subject)
    \addplot[color=blue2,
    solid,
    line width=1pt,
    mark=triangle*,
    mark options={solid},
    mark size=2.5pt] coordinates {
    (1.0,0.081059)(2.0,0.078733)(3.0,0.076383)(4.0,0.074044)
};
    \addlegendentry{2 between + 2 outside}
    \addplot[color=blue2,
    solid,
    line width=1pt,
    mark=none,
    mark options={solid},
    mark size=2.5pt, forget plot] coordinates {
    (4.0,0.074044)(5.0,0.071767)(6.0,0.069628)(7.0,0.067739)(8.0,0.066262)(9.0,0.065437)(10.0,0.065616)
};
    \addplot[only marks, 
    mark=triangle*,color=blue2,mark size=2.5pt,
    line width=1pt, forget plot] coordinates {
     (4.0,0.074044)(5.0,0.071767)(6.0,0.069628)(7.0,0.067739)(8.0,0.066262)(10.0,0.065616) (11.0,0.064627)
    };        
    %plot the minimum
    \addplot[only marks, 
    mark=star,color=blue2,
    mark size=4pt,
    line width=1pt, forget plot] coordinates {
     (9.0,0.065437)
    };       

    
    % 2 bet (1 subject) + 2 outside (1 subject)
    \addplot[color=blue1,
    solid,
    line width=1pt,
    mark=square*,
    mark options={solid},
    mark size=2.5pt] coordinates {
        (1.0,0.073495)(2.0,0.071295)(3.0,0.069078)(4.0,0.066880)
    };
    \addlegendentry{(2) between + (2) outside}    
    \addplot[color=blue1,
    solid,
    line width=1pt,
    mark=none,
    mark options={solid},
    mark size=2.5pt,forget plot] coordinates {
        (4.0,0.066880)(5.0,0.064757)(6.0,0.062788)(7.0,0.061094)(8.0,0.059847)(9.0,0.059309)(10.0,0.059863)
    };
    \addplot[only marks, 
    mark=square*,
    color=blue1,mark size=2.5pt,
    line width=1pt, forget plot] coordinates {
    (4.0,0.066880)(5.0,0.064757)(6.0,0.062788)(7.0,0.061094)(8.0,0.059847)(10.0,0.059863) (11.0,0.062270)
    };        
    %plot the minimum
    \addplot[only marks, 
    mark=star,
    color=blue1,mark size=4pt,
    line width=1pt, forget plot] coordinates {
     (9.0,0.059309)
    };        

        % 3 bet + 1 outside 
    \addplot[color=pink2,
    solid,
    line width=1pt,
    mark=*,
    mark options={solid},
    mark size=2.5pt] coordinates {
    (1.0,0.042011)(2.0,0.040605)(3.0,0.039272)(4.0,0.038066)
};
    \addlegendentry{3 between + 1 outside}
    \addplot[color=pink2,
    solid,
    line width=1pt,
    mark=none,
    mark options={solid},
    mark size=2.5pt,forget plot] coordinates {
(4.0,0.038066)(5.0,0.037068)(6.0,0.036388)(7.0,0.036191)(8.0,0.036708)(9.0,0.038279)(10.0,0.041389)
};
    \addplot[only marks, 
    mark=*,
    color=pink2, mark size=2.5pt,
    line width=1pt, forget plot] coordinates {
    (4.0,0.038066)(5.0,0.037068)(6.0,0.036388)(8.0,0.036708)(9.0,0.038279)(10.0,0.041389) (11.0,0.044872)
    };  
     %plot the minimum
    \addplot[only marks, 
    mark=star,
    color=pink2, mark size=4pt,
    line width=1pt, forget plot] coordinates {
     (7.0,0.036191)
    };         
    
    %4 pbrn
    \addplot[color=pink1,
    solid,
    line width=1pt,
    mark=diamond*,
    mark options={solid},
    mark size=2.5pt] coordinates {
        (1.0,0.040653) (2.0,0.039561) (3.0,0.038663) (4.0,0.038029)
    };
    \addlegendentry{4 perfect BRN}  
    \addplot[color=pink1,
    solid,
    line width=1pt,
    mark=none,
    mark options={solid},
    mark size=2.5pt,forget plot] coordinates {
       (4.0,0.038029) (5.0,0.037751) (6.0,0.037944) (7.0,0.038765) (8.0,0.040412) (9.0,0.043149) (10.0,0.047313) 
    };
    \addplot[only marks, 
    mark=diamond*,
    color=pink1,mark size=2.5pt,
    line width=1pt, forget plot] coordinates {
     (4.0,0.038029) (6.0,0.037944) (7.0,0.038765) (8.0,0.040412) (9.0,0.043149) (10.0,0.047313) (11.0,0.053698) 
    };  
    %plot the minimum
    \addplot[only marks, 
    mark=star,
    color=pink1,mark size=4pt,
    line width=1pt, forget plot] coordinates {
     (5.0,0.037751)
    };  

    % 4bet
    \addplot[color=pink3,
    solid,
    line width=1pt,
    mark=triangle,
    mark options={solid},
    mark size=2.5pt] coordinates {
        (1.0,0.009040) (2.0,0.008260) (3.0,0.007597) (4.0,0.007126) 
    };
    \addlegendentry{4 between}
    \addplot[color=pink3,
    solid,
    line width=1pt,
    mark=none,
    mark options={solid},
    mark size=2.5pt,forget plot] coordinates {
         (4.0,0.007126) (5.0,0.006950) (6.0,0.007221) (7.0,0.008164) (8.0,0.010105) (9.0,0.013520) (10.0,0.019098)
    };
    \addplot[only marks, 
    mark=triangle,
    color=pink3,mark size=2.5pt,
    line width=1pt, forget plot] coordinates {
      (6.0,0.007221) (7.0,0.008164) (8.0,0.010105) (9.0,0.013520) (10.0,0.019098)(11.0,0.024908)
    };    
     %plot the minimum
    \addplot[only marks, 
    mark=star,
    color=pink3,mark size=4pt,
    line width=1pt, forget plot] coordinates {
      (5.0,0.006950)
    };    
    


    
    %4 bayese
    \addplot[color=pink4,
    solid,
    line width=1pt,
    mark=diamond,
    mark options={solid},
    mark size=2.5pt] coordinates {
        (1.0,0.024491)(2.0,0.022494)(3.0,0.020381)(4.0,0.018164)
    };
    \addlegendentry{4 perfect Bayes}
    \addplot[color=pink4,
    solid,
    line width=1pt,
    mark=none,
    mark options={solid},
    mark size=2.5pt,forget plot] coordinates {
        (4.0,0.018164)(5.0,0.015874)(6.0,0.013572)(7.0,0.011372)(8.0,0.009475)(9.0,0.008238)(10.0,0.008287)
    };
    \addplot[only marks, 
    mark=diamond,
    color=pink4,mark size=2.5pt,
    line width=1pt, forget plot] coordinates {
     (4.0,0.018164)(5.0,0.015874)(6.0,0.013572)(7.0,0.011372)(8.0,0.009475)(9.0,0.008238) (11.0,0.009934)
    };  
     %plot the minimum
    \addplot[only marks, 
    mark=star,
    color=pink4,mark size=4pt,
    line width=1pt, forget plot] coordinates {
      (10.0,0.008287)
    };     



    
    \end{axis}
\end{tikzpicture}
    \caption{Aggregator Performance in Subsample}
    \label{fig: classical_regrets}
\end{figure}
